Benchmarking Simulation-Based Inference

Recent advances in probabilistic modelling have led to a large number of simulation-based inference algorithms which do not require numerical evaluation of likelihoods. However, a public benchmark with appropriate performance metrics for such 'likelihood-free' algorithms has been lacking. This has made it difficult to compare algorithms and identify their strengths and weaknesses. We set out to fill this gap: We provide a benchmark with inference tasks and suitable performance metrics, with an initial selection of algorithms including recent approaches employing neural networks and classical Approximate Bayesian Computation methods. We found that the choice of performance metric is critical, that even state-of-the-art algorithms have substantial room for improvement, and that sequential estimation improves sample efficiency. Neural network-based approaches generally exhibit better performance, but there is no uniformly best algorithm. We provide practical advice and highlight the potential of the benchmark to diagnose problems and improve algorithms. The results can be explored interactively on a companion website. All code is open source, making it possible to contribute further benchmark tasks and inference algorithms.

==> figs/_algorithms_tikz_source/_styles.tex <==
%
% Font
%
%\tikzset{font={\fontsize{22pt}{22}\selectfont}}
\tikzset{font={\fontsize{22pt}{22}\fontfamily{phv}\selectfont}}

%
% Colors
%
\tikzstyle{light_bg} = [fill=white]
\tikzstyle{gray_bg} = [fill=black!5]

%
% Distances
%
\tikzstyle{dist_normal} = [node distance = 2.5cm]
\tikzstyle{dist_large} = [node distance = 3.5cm]
\tikzstyle{dist_xlarge} = [node distance = 4.5cm]
\tikzstyle{dist_xxlarge} = [node distance = 6.8cm]

%
% Title
%
%\tikzstyle{title} = [text width=30em, text centered, minimum height=5em, font={\fontsize{28pt}{28}\selectfont}]
\tikzstyle{title} = [text width=30em, text centered, minimum height=5em, font={\fontsize{26pt}{32}\fontfamily{phv}\selectfont}]

%
% Boxes
%
\tikzstyle{block} = [rectangle, draw, fill=white, 
    text width=10em, text centered, rounded corners, minimum height=5em, dist_normal]
\tikzstyle{prior} = [light_bg]
\tikzstyle{proposal} = [light_bg]
\tikzstyle{posterior} = [light_bg]
\tikzstyle{data} = []
\tikzstyle{simulator} = [text width=14em, minimum height=5em, fill=black, text=white]
\tikzstyle{model} = [gray_bg, text width=14em, minimum height=5em]
\tikzstyle{decision} = [diamond, draw, fill=white, 
    text width=9.5em, text badly centered, inner sep=0pt, dist_large]

%
% Arrows
%
\tikzstyle{line_plain} = [draw, -]
\tikzstyle{line_arrow} = [draw, -{Latex[length=3mm,width=4mm]}]



==> figs/_algorithms_tikz_source/figure.tex <==
\begin{figure*}[t]
    \centering
    %
    \input{figs/tikz/_styles}
    %
    \begin{subfigure}[htbp]{0.245\textwidth}
        \resizebox{!}{4cm}{
            \trimbox{-2cm 0cm 0cm 0cm}{ 
                \input{figs/tikz/monte_carlo-abc}
            }
        }
    \end{subfigure}
    %
    \begin{subfigure}[htbp]{0.245\textwidth}
        \resizebox{!}{4cm}{
            \trimbox{0cm 0cm 0cm 0cm}{
                \input{figs/tikz/likelihood_estimation}
            }
        }
    \end{subfigure}
    %
    \begin{subfigure}[htbp]{0.245\textwidth}
        \resizebox{!}{4cm}{
            \trimbox{-2cm 0cm 0cm 0cm}{
                \input{figs/tikz/posterior_estimation}
            }
        }
    \end{subfigure}
    %
    \begin{subfigure}[htbp]{0.245\textwidth}
        \resizebox{!}{4cm}{
            \trimbox{0cm 0cm 0cm 0cm}{
                \input{figs/tikz/ratio_estimation}
            }
        }
    \end{subfigure}
    %
    \caption{
        {\bf Overview of algorithms.} We compare eight different algorithms for simulation-based inference: \ABC{}, \SABC{}, \NLE{}, \SNLE{}, \NPE{}, \SNPE{}, \NRE{} and \SNRE{}. These algorithms represent distinct approaches to SBI, which are reflected in our naming scheme. Classification and schemes following \cite{cranmer2019}. 
    }
    %
    \label{fig:algorithms}
    %
    %
\end{figure*}


==> figs/_algorithms_tikz_source/likelihood_estimation.tex <==
\begin{tikzpicture}[node distance = 2.5cm, auto]
    %
    % Nodes
    %
    \node [title] (title) {\color{NLE}{Likelihood Estimation}};
    \node [block, proposal, below of=title] (proposal) {proposal};
    \node [block, prior, left of=proposal, dist_xlarge] (prior) {prior};
    \node [block, simulator, below of=proposal] (simulator) {simulator};
    \node [block, model, below of=simulator] (model) {likelihood estimator};
    \node [decision, below of=model] (decision) {infer};
    \node [block, data, right of=decision, dist_xlarge] (data) {data};
    \node [block, posterior, below of=decision, dist_large] (posterior) {posterior};
    %
    % Extra coordinates
    %
    \coordinate [right of=simulator, dist_xxlarge] (c1);
    %
    % Edges
    %
    \path [line_arrow] (prior) -- (proposal);
    \path [line_arrow] (prior) |- (decision);
    \path [line_arrow] (proposal) -- (simulator);
    \path [line_arrow] (simulator) -- (model);
    \path [line_arrow] (model) -- (decision);
    \path [line_arrow] (data) -- (decision);
    \path [line_plain,dashed] (posterior) -| (c1);
    \path [line_arrow,dashed] (c1) |- (proposal);
    \path [line_arrow] (decision) -- (posterior);
    %
    % Sequential label
    %
    \node [rotate=90] at (7.7, -8.) {\color{SNLE}{sequential}};
\end{tikzpicture}


==> figs/_algorithms_tikz_source/monte_carlo-abc.tex <==
\begin{tikzpicture}[auto]
    %
    % Nodes
    %
    \node [title] (title) {\color{SABC}{Monte Carlo ABC}};
    \node [block, prior, below of=title] (prior) {prior};
    \node [block, proposal, below of=prior] (proposal) {proposal};
    \node [block, simulator, below of=proposal] (simulator) {simulator};
    \node [decision, below of=simulator] (decision) {compare};
    \node [block, data, dist_xlarge, left of=decision] (data) {data};
    \node [block, posterior, dist_large, below of=decision] (posterior) {posterior};
    %
    % Extra coordinates
    %
    \coordinate [dist_large, right of=simulator] (c1);
    %
    % Edges
    %
    \path [line_arrow] (prior) -- (proposal);
    \path [line_arrow] (proposal) -- (simulator);
    \path [line_arrow] (simulator) -- (decision);
    \path [line_arrow] (data) -- (decision);
    \path [line_plain,dashed] (decision) -| (c1);
    \path [line_arrow,dashed] (c1) |- (proposal);
    \path [line_arrow] (decision) -- (posterior);
    %
    % Sequential label
    %
    \node [rotate=90] at (4.3, -8.) {\color{SABC}{sequential}};
\end{tikzpicture}

==> figs/_algorithms_tikz_source/posterior_estimation.tex <==
\begin{tikzpicture}[node distance = 2.5cm, auto]
    %
    % Nodes
    %
    \node [title] (title) {\color{SNPE}{Posterior Estimation}};
    \node [block, proposal, below of=title] (proposal) {proposal};
    \node [block, prior, left of=proposal, dist_xlarge] (prior) {prior};
    \node [block, simulator, below of=proposal] (simulator) {simulator};
    \node [block, model, below of=simulator] (model) {posterior estimator};
    \node [decision, below of=model] (decision) {evaluate};
    \node [block, data, left of=decision, dist_xlarge] (data) {data};
    \node [block, posterior, below of=decision, dist_large] (posterior) {posterior};
    %
    % Extra coordinates
    %
    \coordinate [right of=simulator, dist_large] (c1);
    %
    % Edges
    %
    \path [line_arrow] (prior) -- (proposal);
    \path [line_arrow] (proposal) -- (simulator);
    \path [line_arrow] (simulator) -- (model);
    \path [line_arrow] (model) -- (decision);
    \path [line_arrow] (data) -- (decision);
    \path [line_plain,dashed] (decision) -| (c1);
    \path [line_arrow,dashed] (c1) |- (proposal);
    \path [line_arrow] (decision) -- (posterior);
    %
    % Sequential label
    %
    \node [rotate=90] at (4.3, -6.8) {\color{SNPE}{sequential}};
\end{tikzpicture}


==> figs/_algorithms_tikz_source/ratio_estimation.tex <==
\begin{tikzpicture}[node distance = 2.5cm, auto]
    %
    % Nodes
    %
    \node [title] (title) {\color{NRE}{Ratio Estimation}};
    \node [block, proposal, below of=title] (proposal) {proposal};
    \node [block, prior, left of=proposal, dist_xlarge] (prior) {prior};
    \node [block, simulator, below of=proposal] (simulator) {simulator};
    \node [block, model, below of=simulator] (model) {ratio estimator};
    \node [decision, below of=model] (decision) {infer};
    \node [block, data, right of=decision, dist_xlarge] (data) {data};
    \node [block, posterior, below of=decision, dist_large] (posterior) {posterior};
    %
    % Extra coordinates
    %
    \coordinate [right of=simulator, dist_xxlarge] (c1);
    %
    % Edges
    %
    \path [line_arrow] (prior) -- (proposal);
    \path [line_arrow] (prior) |- (decision);
    \path [line_arrow] (proposal) -- (simulator);
    \path [line_arrow] (simulator) -- (model);
    \path [line_arrow] (model) -- (decision);
    \path [line_arrow] (data) -- (decision);
    \path [line_plain,dashed] (posterior) -| (c1);
    \path [line_arrow,dashed] (c1) |- (proposal);
    \path [line_arrow] (decision) -- (posterior);
    %
    % Sequential label
    %
    \node [rotate=90] at (7.7, -8.) {\color{SNRE}{sequential}};
\end{tikzpicture}


==> figs/_algorithms_tikz_source/tikz.tex <==
\input{style/aistats2021}
% main document, called main.tex
\input{preamble/preamble}
\usepackage{tikz}
\usetikzlibrary{external}
\tikzexternalize % activate!
\begin{document}
\input{figs/tikz/figure}
\end{document}
